Computing Nash Equilibria in Potential Games with Private Uncoupled Constraints

We consider the problem of computing Nash equilibria in potential games where each player's strategy set is subject to private uncoupled constraints. This scenario is frequently encountered in real-world applications like road network congestion games where individual drivers adhere to personal budget and fuel limitations. Despite the plethora of algorithms that efficiently compute Nash equilibria (NE) in potential games, the domain of constrained potential games remains largely unexplored. We introduce an algorithm that leverages the Lagrangian formulation of NE. The algorithm is implemented independently by each player and runs in polynomial time with respect to the approximation error, the sum of the size of the action-spaces, and the game's inherent parameters.

==> extras.tex <==
\begin{definition}[Primal problem - per player]
\label{def:primal_per_player}
Let each player $i \in [n]$ have a set of $C_i$ private constraints, denoted by $g^{(m)}_{i}(\cdot)$ for any $m \in [C_i]$. Then, given a fixed joint strategy profile for the other players $\bm{\hat{x}}_{-i}$, player $i$ aims to solve the following optimization problem.

\begin{equation} \label{eq:primal_per_player}
\begin{array}{ccc}
  \text{minimize}   & \Phi(\bm{x}_i, \bm{\hat{x}}_{-1}) & \\
  \text{subject to} & g^{(m)}_i(\bm{x}_i) \leq 0, & m = 1, 2, \ldots, C_i \\
\end{array}
\end{equation}

\end{definition}

The main concept of the Lagrangian method is to create a modified problem that includes the constraints. In particular, for each player, we start with the primal problem given in \cref{def:primal_per_player}, and then construct a new problem using the Lagrangian method.

\begin{definition}[Dual problem - per player]
\label{def:dual_per_player}
Let $i \in [n]$ be an arbitrary player associated with a primal problem, as defined in \cref{def:primal_per_player}. Then, the dual (Lagrangian) problem is defined as follows.

\begin{equation} \label{eq:dual_per_player}
\begin{array}{ccc}
  \text{maximize}   & \inf\limits_{\bm{x}_i \in \Delta(\mathcal{A}_i)} \mathcal{L}_i(\bm{x}_i, \bm{\lambda}_i; \bm{\hat{x}}_{-1}) & \\
  \text{subject to} & \bm{\lambda}_i \succeq \bm{0}
\end{array}
\end{equation}

where $
\mathcal{L}_i(\bm{x}_i, \bm{\lambda}_i; \bm{\hat{x}}_{-1}) 
\coloneqq 
\Phi(\bm{x}_i, \bm{\hat{x}}_{-i})
+ 
\sum\limits_{m=1}^{C_i} \lambda_i^{(m)} g_{i}^{(m)}(\bm{x}_i)
$ and $\bm{\lambda}_i \in \mathbb{R}^{C_i}_{+}$.
\end{definition}

\subsubsection{Our goal}
The goal is to find a pair $(\bm{\hat{x}}_i, \bm{\hat{\lambda}}_i)$ for each player $i \in [n]$, that is a approximate Nash equilibrium. However, in cases where the the optimization is being done over a specific convex domain the notion of Nash equilibrium




\begin{lemma} \label{lemma:unique_maximizer}
Let $\bm{\hat{x}}$ be an arbitrary joint strategy profile. Then, for any player $i \in [n]$ the function $\mathcal{L}_i (\bm{\hat{x}_i}, \bm{\lambda}_i ; \bm{\hat{x}_{-i}}) - \mu \norm{\bm{\lambda}_i}^2 = \mathcal{\Tilde{L}}_i(\bm{\hat{x}_{i}}, \bm{\lambda}_i; \bm{\hat{x}_{-i}})$ is strongly concave, and so the maximizer $\bm{\hat{\lambda}_i} = \arg \max_{\bm{\lambda}_i} \{ \mathcal{\Tilde{L}}_i(\bm{\hat{x}}, \bm{\lambda}_i) \} $ is unique.
\end{lemma}

\begin{proof}
Since the Lagrangian $\mathcal{L}(\bm{\hat{x}_i}, \bm{\lambda}_i ; \bm{\hat{x}_{-i}})$ is linear in $\bm{\lambda}_i$ to prove that the regularized Lagrangian $\mathcal{\Tilde{L}}_i(\bm{\hat{x}_{i}}, \bm{\lambda}_i; \bm{\hat{x}_{-i}})$ is strongly concave, it suffices to prove that the regularization term, $\mu \norm{\lambda}^2$, is strongly concave. It can be easily shown that $h(\bm{\lambda}) = \mu \norm{\bm{\lambda}}^2$ is strongly concave, as the Hessian matrix $\nabla^2 h(\bm{\lambda}) = 2 \mu I^{n \times n}$ is positive definite.

Regarding the uniqueness of the maximizer, it readily follows as a strongly concave function is necessarily strictly concave as well.
\end{proof}

\begin{lemma} \label{lemma:bounded_maximizer}
Let $\bm{\hat{x}}$ be an arbitrary joint strategy profile. Then, for any player $i \in [n]$ the maximizer $\bm{\hat{\lambda}_i} = \arg \max_{\bm{\lambda}_i} \{ \mathcal{\Tilde{L}}_i(\bm{\hat{x}}, \bm{\lambda}_i) \} $ is bounded above by $\frac{G^{\textrm{MAX}}_i}{2 \mu}$.
\end{lemma}

\begin{proof}
Let $\bm{\hat{\lambda}_i}$ be the maximizer of $\mathcal{\Tilde{L}}_i(\bm{\hat{x}}, \cdot)$. According to \cref{lemma:unique_maximizer}, we know that $\bm{\hat{\lambda}_i}$ is unique and that the gradient of $\mathcal{\Tilde{L}}_i(\bm{\hat{x}}, \cdot)$ with respect to $\bm{\lambda}_i$ must vanish at $\bm{\hat{\lambda}_i}$.

\begin{align}
\nabla_{\bm{\lambda}} 
\left(
\mathcal{\Tilde{L}}_i(\bm{\hat{x}}, \bm{\hat{\lambda}}_i)
\right)
=
\nabla_{\bm{\lambda}} 
\left(
\Phi(\hat{\bm{x}}) + 
\sum\limits_{m=1}^{C_i}
\lambda_i^{(m)} g^{(m)}(\bm{\hat{x}}_i) - \ell \norm{\bm{\lambda}_i}^2
\right)
=
\bm{0}
\end{align}

Then, for any constraint $m \in \{ 1, 2, \ldots, C_i \}$ it follows that

\begin{align}
\frac{\partial}{\partial \lambda^{(m)}_{i}}
\left(
\mathcal{\Tilde{L}}_i(\bm{\hat{x}}, \bm{\hat{\lambda}}_i)
\right)
=
g^{(m)}_{i} (\bm{\hat{x}}_i) + 2 \mu \lambda^{(m)}_{i} = 0 
\Rightarrow
\lambda^{(m)}_{i} 
=
\frac{g^{(m)}_{i} (\bm{\hat{x}}_i)}{2 \mu}
\leq
\frac{G^{\textrm{MAX}}_i}{2 \mu}
\end{align}

where $G^{\textrm{MAX}}_i = \max\limits_{\bm{x}_i \in \Delta(\mathcal{A}_i)} \max\limits_{m \in [C_i]} g^{(m)}_i(\bm{\hat{x}}_i)$ is the maximum value over all $\bm{x}_i \in \Delta(\mathcal{A}_i)$ and over all constraints of player $i$. 

\end{proof}

\begin{lemma}
Suppose $\pxhat$ is a stationary point of $g(\hat{x}, \lambda)$. Then, it is uniquely extended to a pair of optimal solutions $(\hat{x}, \lambda)$ of the Lagrangian function $\mathcal{L}(\hat{x},\hat{\lambda})$.
\end{lemma}
\begin{proof}
The reason for this extensibility argument depends on the fact that the regularized function $g(\hat{x},\lambda)$ is strongly-concave, and so the maximizer is uniquely determined. 
\end{proof}


\begin{lemma}
Suppose $\pxhat$ is a stationary point of $g(\hat{x}, \lambda)$. Then, it is uniquely extended to a pair of optimal solutions $(\hat{x}, \lambda)$ of the Lagrangian function $\mathcal{L}(\hat{x},\hat{\lambda})$.
\end{lemma}
\begin{proof}
The reason for this extensibility argument depends on the fact that the regularized function $g(\hat{x},\lambda)$ is strongly-concave, and so the maximizer is uniquely determined. 
\end{proof}

==> nonconvex_games/nonconvex_figure.tex <==
\begin{figure}[!ht]
    \centering
    \input{}
    \caption{Nonconvex feasibility set}
    \label{fig:nonconcave_constraints}
\end{figure}

